When Fair Ranking Meets Uncertain Inference

Existing fair ranking systems, especially those designed to be demographically fair, assume that accurate demographic information about individuals is available to the ranking algorithm. In practice, however, this assumption may not hold -- in real-world contexts like ranking job applicants or credit seekers, social and legal barriers may prevent algorithm operators from collecting peoples' demographic information. In these cases, algorithm operators may attempt to infer peoples' demographics and then supply these inferences as inputs to the ranking algorithm. In this study, we investigate how uncertainty and errors in demographic inference impact the fairness offered by fair ranking algorithms. Using simulations and three case studies with real datasets, we show how demographic inferences drawn from real systems can lead to unfair rankings. Our results suggest that developers should not use inferred demographic data as input to fair ranking algorithms, unless the inferences are extremely accurate.

==> Makefile <==
# Tools
LATEXMK = latexmk
RM = rm -f
PYTHON = python3

# Project-specific settings
DOCNAME = main
PLOTDIR = ../plots/
TEXFILES = $(wildcard *.tex)

# Targets
all: doc
doc: pdf
pdf: $(DOCNAME).pdf

# Rules
figures:

tables:


%.pdf: $(TEXFILES)
#	$(LATEXMK) -pdf -M -MP -MF $*.d $*
	pdflatex $(DOCNAME).tex
	bibliography/run-crosstex $(DOCNAME)
	pdflatex $(DOCNAME).tex
	pdflatex $(DOCNAME).tex

paperclean:
	$(LATEXMK) -silent -C
	$(RM) *.run.xml *.synctex.gz
	$(RM) *.d
	$(RM) *.bbl	

mostlyclean:
	$(LATEXMK) -silent -c
	$(RM) *.bbl

clean: mostlyclean
	$(LATEXMK) -silent -C
	$(RM) *.run.xml *.synctex.gz
	$(RM) *.d
	$(RM) $(PLOTDIR)*.pdf

.PHONY: all clean doc mostlyclean pdf

diff: cscw_out.pdf
	cp cscw_out.tex cscw_out.tmp.tex
	perl -pi -e 's/Bibliography\/all/main/g' cscw_out.tmp.tex
	./striptex cscw_out.tmp.tex > current.tex
	latexdiff submission_cscw.tex current.tex > diff.tex
	pdflatex diff.tex
	pdflatex diff.tex
	rm current.tex diff.tex diff.aux diff.log cscw_out.tmp.tex


# Include auto-generated dependencies
-include *.d

